Together We Go Further: LLMs and IDE Static Analysis for Extract Method Refactoring

Long methods that encapsulate multiple responsibilities within a single method are challenging to maintain. Choosing which statements to extract into new methods has been the target of many research tools. Despite steady improvements, these tools often fail to generate refactorings that align with developers' preferences and acceptance criteria. Given that Large Language Models (LLMs) have been trained on large code corpora, if we harness their familiarity with the way developers form functions, we could suggest refactorings that developers are likely to accept. In this paper, we advance the science and practice of refactoring by synergistically combining the insights of LLMs with the power of IDEs to perform Extract Method (EM). Our formative study on 1752 EM scenarios revealed that LLMs are very effective for giving expert suggestions, yet they are unreliable: up to 76.3% of the suggestions are hallucinations. We designed a novel approach that removes hallucinations from the candidates suggested by LLMs, then further enhances and ranks suggestions based on static analysis techniques from program slicing, and finally leverages the IDE to execute refactorings correctly. We implemented this approach in an IntelliJ IDEA plugin called EM-Assist. We empirically evaluated EM-Assist on a diverse corpus that replicates 1752 actual refactorings from open-source projects. We found that EM-Assist outperforms previous state of the art tools: EM-Assist suggests the developerperformed refactoring in 53.4% of cases, improving over the recall rate of 39.4% for previous best-in-class tools. Furthermore, we conducted firehouse surveys with 16 industrial developers and suggested refactorings on their recent commits. 81.3% of them agreed with the recommendations provided by EM-Assist.

==> sections/03-internals.tex <==
\section{internals\label{sec:internals}}

\secpart{Overview}
Use this command to easily switch between proper subsections and simple bold text (which can help to save some space before the deadline).




==> sections/04_RQ4.tex <==
% \subsection{\textbf{RQ4: Runtime performance of \tool}}
% We evaluate our tool's runtime performance to assess its suitability for seamless integration into the developer workflow, ensuring that it incurs minimal overhead.

% \subsubsection{\textbf{Data and Experimental setup}}
% To answer this question, we use the same data set as in \Cref{sec:rq1}, which other researchers used to evaluate their tool. 
% For this analysis, we used the same dataset as discussed in \Cref{sec:rq1}, a dataset commonly employed by previous researchers to evaluate their tools. Our methodology involved executing the tool on all the long methods within the dataset, generating suggestions, and subsequently applying the refactoring to the codebase. 
% We analyzed three key aspects of the process: 
% 1) the time taken to generate the suggestions, 
% 2) the time required to apply the suggestions, and 
% 3) the total time encompassing both suggestion generation and application.
% the following specifications:
% \todo{Intel Core i7-3770 CPU @3.40GHz, 16 GB DDR3 memory, 256GB SSD, MacOS, and Java 11.04 x64.}
% Given that our tool relies on remote LLM invocation via APIs, which is dependent on network speed, we took care to perform the experiments at four different times of the day, ensuring even spacing to account for potential network variability. Conducting experiments at different times of the day helps assess the robustness of a tool by capturing variations in network conditions. 
% It also provides insights into how the tool's performance may align with real-world usage patterns.

% \subsubsection{\textbf{Results}}

